Improving Chest X-Ray Report Generation by Leveraging Warm Starting

Automatically generating a report from a patient's Chest X-Rays (CXRs) is a promising solution to reducing clinical workload and improving patient care. However, current CXR report generators -- which are predominantly encoder-to-decoder models -- lack the diagnostic accuracy to be deployed in a clinical setting. To improve CXR report generation, we investigate warm starting the encoder and decoder with recent open-source computer vision and natural language processing checkpoints, such as the Vision Transformer (ViT) and PubMedBERT. To this end, each checkpoint is evaluated on the MIMIC-CXR and IU X-Ray datasets. Our experimental investigation demonstrates that the Convolutional vision Transformer (CvT) ImageNet-21K and the Distilled Generative Pre-trained Transformer 2 (DistilGPT2) checkpoints are best for warm starting the encoder and decoder, respectively. Compared to the state-of-the-art ($\mathcal{M}^2$ Transformer Progressive), CvT2DistilGPT2 attained an improvement of 8.3\% for CE F-1, 1.8\% for BLEU-4, 1.6\% for ROUGE-L, and 1.0\% for METEOR. The reports generated by CvT2DistilGPT2 have a higher similarity to radiologist reports than previous approaches. This indicates that leveraging warm starting improves CXR report generation. Code and checkpoints for CvT2DistilGPT2 are available at https://github.com/aehrc/cvt2distilgpt2.

==> tex/old_cxr_report_generatoin_section.tex <==

\subsection{Old CXR report generation}

In this section, we summarise automatic CXR report generation approaches in the literature. For a more exhaustive review of CXR report generation, we refer the reader to the survey conducted by Kaur \textit{et al.} \cite{Kaur_2021}. As highlighted by Pavlopoulos \textit{et al.}, the two datasets that are consistently used in the literature to evaluate CXR report generation include MIMIC-CXR and IU X-Ray \cite{Pavlopoulos_2021}, which are described in Section \ref{sec:dataset}. The following approaches are evaluated using at least one or both of these datasets.

Wang \textit{et al.} was the first to use an end-to-end encoder-to-decoder model for CXR report generation---a {\small ResNet-50}{\large 2}{\small RNN} with attention, where RNN refers to Recurrent Neural Network.\footnote{Henceforth, the naming convention for encoder-to-decoder models will be the name of the encoder, followed by {\normalsize 2}, followed by the name of the decoder. For example, a model with a CNN encoder and an RNN decoder will be named {\footnotesize CNN}{\normalsize 2}{\footnotesize RNN}.} The authors employed multi-task learning of CXR report generation (IU X-Ray) and multi-label abnormality classification (ChestX-ray14 abnormality labels \cite{Wang_2018}). The ResNet was warm-started using an ImageNet-1K checkpoint. The proposed approach outperformed a general-domain image captioning approach, where several NLG metrics were used for evaluation. However, many type I and II abnormality prediction errors were evident in the generated reports \cite[Figure 4]{Wang_2018}. 

Jing \textit{et al.} also used multi-task learning of CXR report generation (IU X-Ray and the Pathology Education Informational Resource (PEIR) Gross dataset \cite{Jing_2018}) and multi-label abnormality classification (the abnormalities were extracted from the reports), but with a {\small VGG19}{\large 2}{\small HRNN}, where VGG19 is a type of CNN and HRNN refers to a Hierarchical RNN \cite{Jing_2018}. A HRNN consists of a sentence and word RNN. The sentence RNN determines the topic for each sentence given the visual features from the encoder, and the word RNN generates the words for each sentence given the topic \cite{Krause_2017}. The proposed approach fed the co-attention between the predicted abnormalities and the visual features as input to the HRNN. It was able to outperform several general-domain image captioning approaches \cite{Jing_2018}.

To generate a sentence of a report, Xue \textit{et al.} made use of the attention between visual features from the encoder and previous sentences from the report. To produce visual features, the authors made used of ResNet-152 warm-started with an ImageNet-1K checkpoint. Again, the proposed approach was able to outperform multiple general-domain image captioning approaches \cite{Xue_2018}. 

Li \textit{et al.} used an agent that chose (for each sentence of the report) to either use an existing template or to generate a new sentence \cite{Li_2018a}. Although not able to attain higher scores for multiple NLG metrics, the authors noted that their reports were longer and had a higher rate of detecting abnormalities than the approach of Jing \textit{et al.} \cite{Jing_2018}. 

Following this, Jing \textit{et al.} focused on generating the impression and findings sections of a CXR report and modelling the differences between sentences concerned with abnormalities and normalities. The authors exploited the relationships between these sections by having a two-stage system. The first stage generates the findings section, which is given as input to the second stage, which generates the impression. Each stage has multiple RNN agents that generate sentences based on whether or not a region in the image contains an abnormality or not \cite{Jing_2019}. The proposed approach was able to outperform the authors previous work \cite{Jing_2018} and the approach proposed by Li \textit{et al.} \cite{Li_2018a}, where NLG metrics were again used for evaluation.

Subsequently, Li \textit{et al.} incorporated expert knowledge into their model via an abnormality graph. Visual features from a DenseNet were fed into the abnormality graph. The DenseNet was warm-started with a CXR checkpoint formed from the CX-CXR and ChestX-Ray8 datasets, where multi-label abnormality classification was the pre-training task \cite{Wang_2018}. The predicted abnormalities were then used to retrieve sentence templates, where the final CXR report was generated based on the selected templates \cite{Li_2019}. This was able to outperform the authors previous approach for a majority of the tested NLG metrics \cite{Li_2018a}. 

While NLG metrics capture the similarity between the predicted and ground truth reports, they do not always capture diagnostic accuracy \cite{Pavlopoulos_2021}. Motivated by this, Liu \textit{et al.} used the CheXpert labeler to form a classification metric; CheXpert is a tool that extracts up to 14 observations from a report (12 of which were abnormalities). Each observation is considered to be either \textit{positive}, \textit{negative}, \textit{uncertain}, or \textit{not mentioned} \cite{Irvin_2019}. Using this, observations are extracted from the generated and ground truth reports. Finally, the scores are given using classification metrics such as precision and recall between the observations of the generated and ground truth reports. Liu \textit{et al.} used the classification scores of CheXpert as the reward for Self-Critical Sequence Training (SCST) \cite{Rennie_2017} to train a {\small ResNet-101}{\large 2}{\small HRNN}, where previously an NLG metric would be the reward \cite{Liu_2019}. SCST enables the decoder to be trained with its own outputs as input---something that is not possible with standard training schema. This is achieved by using a reinforcement learning algorithm, which uses the score between the generated and ground truth reports as the reward. Again, the encoder was warm-started using an ImageNet-1K checkpoint. This was able to outperform the approach by Wang \textit{et al.} for all tested NLG metrics \cite{Wang_2018}. It was also demonstrated that using the classification scores of CheXpert as the reward with SCST improves the diagnostic accuracy of the generated reports.

Xiong \textit{et al.} incorporated an object detector into the encoder---to produce visual features based on regions of interest. DenseNet-121 warm-started with a ChestX-Ray14 checkpoint was the backbone of the object detector. A Transformer was used as the decoder, where SCST helped improve the coherence of the reports. This was able to outperform multiple approaches that used an RNN as the decoder \cite{Xiong_2019, Wang_2017}. 

Huang \textit{et al.} employed an HRNN whose input is based on the attention of the channel and spatial information of the visual features. Differing from previous approaches, the word RNN takes the topics and an embedding of the patient's background information as input. ResNet-152 warm-started with an ImageNet-1K checkpoint was used as the encoder \cite{Huang_2019}. This outperformed the approach of Jing \textit{et al.}, where several NLG metrics and a metric based on Medical Subject Heading (MeSH) terms were used for evaluation \cite{Jing_2018}. 

Yuan \textit{et al.} employed multi-task learning of multi-label abnormality classification and CXR report generation and a {\small ResNet-152}{\large 2}{\small HRNN}. The encoder was warm-started using a CheXpert checkpoint \cite{Irvin_2019}. Moreover, a separate sentence RNN was applied to the visual features. Attention was also applied to the visual features and the predicted abnormalities \cite{Yuan_2019}. This was able to outperform the approaches of Jing \textit{et al.} and Li \textit{et al.}, where multiple NLG metrics were used for evaluation \cite{Jing_2018, Li_2018a}. 

To embed expert knowledge, Zhang \textit{et al.} incorporated a Graph Convolutional Network (GCN)---whose nodes consisted of abnormalities---into the encoder \cite{Zhang_2020}. This was able to outperform several of the aforementioned CXR report generation approaches, where multiple NLG metrics were used for evaluation \cite{Wang_2018, Jing_2018, Li_2018a, Liu_2019, Yuan_2019}. The authors also developed a diagnostic accuracy metric based on the graph CNN---which was used to determine that the graph CNN is able to increase diagnostic accuracy.

More recently, Lovelace and Mortazavi employed a CNN followed by a series of Transformer layers as the encoder and a Transformer decoder. To improve diagnostic accuracy, CheXpert was used to extract observations from the generated report in a differentiable manner, where the loss between the observations of the generated and ground truth reports was added to the training loss. This outperformed multiple approaches that employed an RNN as the decoder, were multiple NLG metrics and CheXpert classification scores were used for evaluation \cite{Lovelace_2020}. 

Chen \textit{et al.} proposed a ``memory-driven" Transformer decoder \cite{Chen_2020}, which later included ``cross-modal memory" \cite{Chen_2021}. Using multiple NLG metrics and the CheXpert classification metric, it was determined that the proposed approaches were able to outperform several of the aforementioned CXR report generation approaches, each of which used an RNN as the decoder \cite{Jing_2019, Li_2018a, Jing_2018}.

Alfarghaly \textit{et al.} employed DenseNet-121 as the encoder and a Transformer as the decoder. DenseNet-121 was warm-started with CheXNet: a ChestX-ray14 checkpoint. The decoder was warm-started with DistilBERT, a general-domain NLG checkpoint. However, cross-attention was not used with each layer of the decoder, rather the embeddings of each predicted abnormality of CheXNet were fed as input to DistilGPT2. In terms of multiple NLG metrics, this method outperformed multiple approaches that utilised an RNN as the decoder \cite{Alfarghaly_2021}.

Liu \textit{et al.} proposed the Contrastive Attention model which compares the current CXR to a pool of CXRs that have no abnormalities. Contrastive Attention comprises two modules, ``aggregate attention" and ``difference attention". Aggregate attention finds the normal CXRs from the pool that are closest to the CXR in question. Difference attention involves two steps; for the first step, common features between the current CXR and the pool of normal CXRs are found. For the second step, the common features are subtracted from the features of the current CXR to capture ``contrastive information". The authors adopt ResNet-50 warm-started with an ImageNet-1K checkpoint that was additionally trained on CheXpert. This was able to outperform the aforementioned ``memory-driven" Transformer proposed by Chen \textit{et al.}, where multiple NLG metrics and the CheXpert classification scores were used for evaluation \cite{Liu_2021a}.

With the aim to imitate the interpretation process of radiologists, Liu \textit{et al.} proposed the \textit{a Posterior}-and-\textit{Prior} Knowledge Exploring-and-Distilling approach (PPKED)  \cite{Liu_2021b}. Along with a CXR, the model consumes embeddings of the most common abnormalities found in the reports from the training set. It also consumes encoded reports from CXRs of the training set that have similar visual features to the current CXR. Finally, the model also consumes the embedding from a knowledge graph that represents the embeddings. The visual features were computed by a ResNet-152 that was warm-started with an ImageNet-1K checkpoint additionally trained on CheXpert. This outperformed the aforementioned ``memory-driven" Transformer proposed by Chen \textit{et al.}, where multiple NLG metrics and the CheXpert classification scores were used for evaluation \cite{Liu_2021a}.

Nooralahzadeh \textit{et al.} proposed an approach that generated a report from detected abnormalities in the CXR \cite{Nooralahzadeh_2021}. First, a DenseNet-121 extracts visual features from a CXR, where a pre-trained CheXpert checkpoint was used for warm-starting. Next, an encoder-to-decoder model called the meshed Transformer with memory ($\mathcal{M}^2$ Transformer) \cite{Cornia_2020} predicted the abnormalities from the visual features. The labels for the $\mathcal{M}^2$ Transformer were extracted from the CXR using the GCN of Zhang \textit{et al.} \cite{Zhang_2020}. These were fed to BART to generate the report, where BART a sequence-to-sequence encoder-to-decoder model \cite{Lewis_2020}. This outperformed the approach of Chen \textit{et al.}, where multiple NLG metrics and the CheXpert classification metric were used for evaluation \cite{Liu_2021a}.

==> tex/table_hyperparameter_search.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}
\centering
\caption{Generated by Spread-LaTeX}\label{tab:hyperparameter_search}
\scriptsize
\begin{tabular}{lrrr}\toprule
Hyperparameter &Interval/set &Log \\\midrule
Resize size &[Image size, image size + 64) & \\
Learning rate (encoder) &[1e-7,1e-2) &\checkmark \\
Learning rate (everything else) &[1e-7,1e-2) &\checkmark \\
Freeze domain-specific parameters &{True, false} & \\
Optimiser &{SGD, Adam, or AdamW} & \\
Warmup steps &[1,1024) & \\
Maximum rotation degrees &$[0^{\circ},10^{\circ})$ & \\
\bottomrule
\end{tabular}
\end{table}

==> tex/table_mimic_cxr_old.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}
\centering
\caption{Mean NLG metric scores on the MIMIC-CXR test set with the labels of Chen \textit{et al.} \cite{Chen_2020}. The highest mean score for each metric is in boldface. If available, the 95\% confidence intervals are reported. $n=5$ indicates the mean over five training runs. * is the training run that scored the highest validation CIDEr score.}\label{tab:mimic_cxr}
% \tiny
\setlength{\tabcolsep}{0pt}

\begin{tabular}{w{l}{41mm} w{r}{9mm} >{\tiny}w{c}{1.5mm} >{\tiny}w{l}{7mm} w{r}{9mm} >{\tiny}w{c}{1.5mm} >{\tiny}w{l}{7mm} w{r}{9mm} >{\tiny}w{c}{1.5mm} >{\tiny}w{l}{7mm} w{r}{9mm} >{\tiny}w{c}{1.5mm} >{\tiny}w{l}{7mm} w{r}{9mm} >{\tiny}w{c}{1.5mm} >{\tiny}w{l}{7mm} w{r}{9mm} >{\tiny}w{c}{1.5mm} >{\tiny}w{l}{7mm} w{r}{9mm} >{\tiny}w{c}{1.5mm} >{\tiny}w{l}{7mm}   }\toprule
\multirow{2}{*}{\textbf{Model}} &\multicolumn{21}{c}{\textbf{Natural language generation metrics}} \\\cmidrule{2-22}
&\multicolumn{3}{c}{\textbf{BLEU-1}} &\multicolumn{3}{c}{\textbf{BLEU-2}} &\multicolumn{3}{c}{\textbf{BLEU-3}} &\multicolumn{3}{c}{\textbf{BLEU-4}} &\multicolumn{3}{c}{\textbf{METOER}} &\multicolumn{3}{c}{\textbf{ROUGE-L}} &\multicolumn{3}{c}{\textbf{CIDER}} \\\midrule
Transformer \cite{Chen_2020} &\cellcolor[HTML]{f8696b}0.3140 &\cellcolor[HTML]{f8696b} &\cellcolor[HTML]{f8696b} &\cellcolor[HTML]{f8696b}0.1920 &\cellcolor[HTML]{f8696b} &\cellcolor[HTML]{f8696b} &\cellcolor[HTML]{f8696b}0.1270 &\cellcolor[HTML]{f8696b} &\cellcolor[HTML]{f8696b} &\cellcolor[HTML]{f8696b}0.0900 &\cellcolor[HTML]{f8696b} &\cellcolor[HTML]{f8696b} &\cellcolor[HTML]{f8696b}0.1250 &\cellcolor[HTML]{f8696b} &\cellcolor[HTML]{f8696b} &\cellcolor[HTML]{f8696b}0.2650 &\cellcolor[HTML]{f8696b} &\cellcolor[HTML]{f8696b} &- & & \\
R2Gen \cite{Chen_2020} &\cellcolor[HTML]{fdd780}0.3530 &\cellcolor[HTML]{fdd780} &\cellcolor[HTML]{fdd780} &\cellcolor[HTML]{fdd27f}0.2180 &\cellcolor[HTML]{fdd27f} &\cellcolor[HTML]{fdd27f} &\cellcolor[HTML]{fdc67c}0.1450 &\cellcolor[HTML]{fdc67c} &\cellcolor[HTML]{fdc67c} &\cellcolor[HTML]{fdcc7e}0.1030 &\cellcolor[HTML]{fdcc7e} &\cellcolor[HTML]{fdcc7e} &\cellcolor[HTML]{fcc57c}0.1420 &\cellcolor[HTML]{fcc57c} &\cellcolor[HTML]{fcc57c} &\cellcolor[HTML]{fcbf7b}0.2770 &\cellcolor[HTML]{fcbf7b} &\cellcolor[HTML]{fcbf7b} &- & & \\
CMN \cite{Chen_2021} &\cellcolor[HTML]{fdd780}0.3530 &\cellcolor[HTML]{fdd780} &\cellcolor[HTML]{fdd780} &\cellcolor[HTML]{fdd27f}0.2180 &\cellcolor[HTML]{fdd27f} &\cellcolor[HTML]{fdd27f} &\cellcolor[HTML]{fdd67f}0.1480 &\cellcolor[HTML]{fdd67f} &\cellcolor[HTML]{fdd67f} &\cellcolor[HTML]{fee382}0.1060 &\cellcolor[HTML]{fee382} &\cellcolor[HTML]{fee382} &\cellcolor[HTML]{fcc57c}0.1420 &\cellcolor[HTML]{fcc57c} &\cellcolor[HTML]{fcc57c} &\cellcolor[HTML]{fdc67d}0.2780 &\cellcolor[HTML]{fdc67d} &\cellcolor[HTML]{fdc67d} &- & & \\
Contrastive Attention \cite{Liu_2021a} &\cellcolor[HTML]{fdce7e}0.3500 &\cellcolor[HTML]{fdce7e} &\cellcolor[HTML]{fdce7e} &\cellcolor[HTML]{fdd680}0.2190 &\cellcolor[HTML]{fdd680} &\cellcolor[HTML]{fdd680} &\cellcolor[HTML]{ffeb84}0.1520 &\cellcolor[HTML]{ffeb84} &\cellcolor[HTML]{ffeb84} &\cellcolor[HTML]{f0e784}0.1090 &\cellcolor[HTML]{f0e784} &\cellcolor[HTML]{f0e784} &\cellcolor[HTML]{cddd82}0.1510 &\cellcolor[HTML]{cddd82} &\cellcolor[HTML]{cddd82} &\cellcolor[HTML]{ffeb84}0.2830 &\cellcolor[HTML]{ffeb84} &\cellcolor[HTML]{ffeb84} &- & & \\
PPKED \cite{Liu_2021b} &\cellcolor[HTML]{ffeb84}0.3600 &\cellcolor[HTML]{ffeb84} &\cellcolor[HTML]{ffeb84} &\cellcolor[HTML]{ffeb84}0.2240 &\cellcolor[HTML]{ffeb84} &\cellcolor[HTML]{ffeb84} &\cellcolor[HTML]{fedb80}0.1490 &\cellcolor[HTML]{fedb80} &\cellcolor[HTML]{fedb80} &\cellcolor[HTML]{fee382}0.1060 &\cellcolor[HTML]{fee382} &\cellcolor[HTML]{fee382} &\cellcolor[HTML]{ffeb84}0.1490 &\cellcolor[HTML]{ffeb84} &\cellcolor[HTML]{ffeb84} &\cellcolor[HTML]{dfe283}0.2840 &\cellcolor[HTML]{dfe283} &\cellcolor[HTML]{dfe283} &- & & \\
$\mathcal{M}^2$ Transformer Progressive \cite{Nooralahzadeh_2021} &\cellcolor[HTML]{afd480}0.3780 &\cellcolor[HTML]{afd480} &\cellcolor[HTML]{afd480} &\cellcolor[HTML]{cedd82}0.2320 &\cellcolor[HTML]{cedd82} &\cellcolor[HTML]{cedd82} &\cellcolor[HTML]{f0e784}0.1540 &\cellcolor[HTML]{f0e784} &\cellcolor[HTML]{f0e784} &\cellcolor[HTML]{ffeb84}0.1070 &\cellcolor[HTML]{ffeb84} &\cellcolor[HTML]{ffeb84} &\cellcolor[HTML]{fdd57f}0.1450 &\cellcolor[HTML]{fdd57f} &\cellcolor[HTML]{fdd57f} &\cellcolor[HTML]{fa9b74}0.2720 &\cellcolor[HTML]{fa9b74} &\cellcolor[HTML]{fa9b74} &- & & \\
CvT-21{\small 2}DistilGPT2 ($n=5$) &\cellcolor[HTML]{71c27c}0.3918 &\cellcolor[HTML]{71c27c}± &\cellcolor[HTML]{71c27c}0.00008 &\cellcolor[HTML]{7ac57d}0.2454 &\cellcolor[HTML]{7ac57d}± &\cellcolor[HTML]{7ac57d}0.00008 &\cellcolor[HTML]{7fc67d}0.1685 &\cellcolor[HTML]{7fc67d}± &\cellcolor[HTML]{7fc67d}0.00008 &\cellcolor[HTML]{7fc67d}0.1236 &\cellcolor[HTML]{7fc67d}± &\cellcolor[HTML]{7fc67d}0.00009 &\cellcolor[HTML]{a6d27f}0.1525 &\cellcolor[HTML]{a6d27f}± &\cellcolor[HTML]{a6d27f}0.00004 &\cellcolor[HTML]{cbdc81}0.2846 &\cellcolor[HTML]{cbdc81}± &\cellcolor[HTML]{cbdc81}0.00007 &\cellcolor[HTML]{f8696b}0.3614 &\cellcolor[HTML]{f8696b}± &\cellcolor[HTML]{f8696b}0.00052 \\
CvT-21{\small 2}DistilGPT2* &\cellcolor[HTML]{6cc17c}0.3928 &\cellcolor[HTML]{6cc17c}± &\cellcolor[HTML]{6cc17c}0.00013 &\cellcolor[HTML]{6bc17c}0.2478 &\cellcolor[HTML]{6bc17c}± &\cellcolor[HTML]{6bc17c}0.00013 &\cellcolor[HTML]{69c07c}0.1713 &\cellcolor[HTML]{69c07c}± &\cellcolor[HTML]{69c07c}0.00013 &\cellcolor[HTML]{67c07c}0.1267 &\cellcolor[HTML]{67c07c}± &\cellcolor[HTML]{67c07c}0.00013 &\cellcolor[HTML]{75c47d}0.1545 &\cellcolor[HTML]{75c47d}± &\cellcolor[HTML]{75c47d}0.00007 &\cellcolor[HTML]{93cc7e}0.2863 &\cellcolor[HTML]{93cc7e}± &\cellcolor[HTML]{93cc7e}0.00012 &\cellcolor[HTML]{63be7b}\textbf{0.3892} &\cellcolor[HTML]{63be7b}± &\cellcolor[HTML]{63be7b}0.00077 \\
\quad \quad + SCST (CIDEr reward) &\cellcolor[HTML]{63be7b}\textbf{0.3948} &\cellcolor[HTML]{63be7b}± &\cellcolor[HTML]{63be7b}0.00013 &\cellcolor[HTML]{63be7b}\textbf{0.2490} &\cellcolor[HTML]{63be7b}± &\cellcolor[HTML]{63be7b}0.00013 &\cellcolor[HTML]{63be7b}\textbf{0.1720} &\cellcolor[HTML]{63be7b}± &\cellcolor[HTML]{63be7b}0.00013 &\cellcolor[HTML]{63be7b}\textbf{0.1272} &\cellcolor[HTML]{63be7b}± &\cellcolor[HTML]{63be7b}0.00013 &\cellcolor[HTML]{63be7b}\textbf{0.1551} &\cellcolor[HTML]{63be7b}± &\cellcolor[HTML]{63be7b}0.00007 &\cellcolor[HTML]{63be7b}\textbf{0.2878} &\cellcolor[HTML]{63be7b}± &\cellcolor[HTML]{63be7b}0.00012 &\cellcolor[HTML]{ffeb84}0.3790 &\cellcolor[HTML]{ffeb84}± &\cellcolor[HTML]{ffeb84}0.00077 \\
\bottomrule
\end{tabular}
\end{table*}
